Certificates and Witnesses for Multi-objective {\omega}-regular Queries in Markov Decision Processes

Multi-objective probabilistic model checking is a powerful technique for verifying stochastic systems against multiple (potentially conflicting) properties. To enhance the trustworthiness and explainability of model checking tools, we present independently checkable certificates and witnesses for multi-objective {\omega}-regular queries in Markov decision processes. For the certification, we extend and improve existing certificates for the decomposition of maximal end components and reachability properties. We then derive mixed-integer linear programs (MILPs) for finding minimal witnessing subsystems. For the special case of Markov chains and LTL properties, we use unambiguous B\"uchi automata to find witnesses, resulting in an algorithm that requires single-exponential space. Existing approaches based on deterministic automata require doubly-exponential space in the worst case. Finally, we consider the practical computation of our certificates and witnesses and provide an implementation of the developed techniques, along with an experimental evaluation, demonstrating the efficacy of our techniques.

==> certificates-reach.tex <==
\section{Certificates for Multi-objective Reachability Queries} 
\label{subsection:multi-reach}
\todo{SJ. I wonder if this should go to the preliminaries, or at least before the first main contribution (EC certificates). It's a bit confusing to mix new contributions with existing work.}



==> compositional.tex <==
\section{Compositionally Determining Witnessing Subsystems}
The \emph{assume-guarantee} framework presented in \cite{kwiatkowska_assume-guarantee_2010} enables the compositional verification of MDPs. We show that their assume-guarantee rules can be repurposed to determine witnessing subsystems in a compositional manner.


==> end-components.tex <==
\section{Certificates for End Components}
For this section, we fix an MDP $\mdp = (\states, \actions, \init, \transMat)$. Now we consider certificates for the MEC decomposition and (non-)existence of satisfying ECs in $\mdp$.
\begin{lemma}[EC-certificate {\cite[Lemma 3.27]{jantsch_certificates_2022}}]
Let $D \subseteq \states$. A \emph{valid EC-certificate} for $D$ is a tuple $(\mathtt{f}, \allowbreak \mathtt{b}) \in \naturals^{D} \times \naturals^{D}$ such that there is a unique $\state^* \in D$ with $\mathtt{f}(\state^*) = \mathtt{b}(\state^*) = 0$ and for each $\state \in \states' \setminus \{\state^*\}$:
\begin{enumerate}[1), align=left, leftmargin=*, itemsep=0mm, topsep=0.8mm, parsep=0mm]
\item $\exists \action \in \actions(\state) \centerdot \mathtt{f}(\state) > \mathtt{f}(\state')\land \transMat(\state, \action, \state') > 0 \land \transMat(\state, \action, D) = 1$.
\item $\exists \state' \in D \centerdot \exists \action' \in \actions(\state) \centerdot \mathtt{b}(\state) > \mathtt{b}(\state') \land \transMat(\state', \action', \state) > 0 \land \transMat(\state', \action', D) = 1$.
\end{enumerate}
\label{def:ec-certificate}
There is an EC with states $D$ in $\mdp$ iff there is a valid EC certificate $(\mathtt{f}, \mathtt{b})$.
\end{lemma}
Intuitively, $\mathtt{f}$ shows that all states in $D$ can reach $\state^*$ and $\mathtt{b}$ that $\state^*$ can reach all states in $D$. Given Rabin properties $\{\pairs_i\}_{i \in [k]}$, this allows us to certify the existence of a satisfying EC in $\mdp$ by returning a valid EC certificate $(\mathtt{f}, \mathtt{b}) \in \naturals^D \times \naturals^D$ with $\Conj_{i=1}^k D \modelsRabin \pairs_i$.
The EC-certificates can also be used to certify the correctness of the \emph{MEC decomposition}. Let $\partition$ be a partition of $\states$. Let $\mecClass[\partition]{\state}$ denote the set $D \in \partition$ that contains $\state$ and $\SA_{\mathcal{D}} = \{(\state,\action) \in \SA \mid \transMat(\state, \action, \mecClass[\partition]{\state}) < 1\}$ the set of pairs that leave their set. Lastly, let $\mathcal{D}_{\MECS}$ be the partitioning of the states according to the MEC they belong to (states $\state$ not belonging to any MEC are put in singletons $\{\state\}$).
\begin{lemma}[MEC-certificate]
A \emph{valid MEC-certificate} for a partition $\partition$ is a tuple $(\mathcal{X}, \vect{r})$ where $\mathcal{X}$ contains \emph{valid EC-certificates} for each $D \in \partition$ and $\vect{r} \in \reals^\states$ with $\vect{A} \vect{r} \geq \vect{1}_{\SA_{\mathcal{D}}}$. Then, $\partition = \partition_{\MECS}$ iff there is a valid MEC certificate for $\mathcal{D}$.
\label{def:mec-certificate}
\end{lemma}
\begin{proof}
By \cite[Lemma~3.27]{jantsch_certificates_2022} we know that each $\ec \in \mathcal{D}$ is an EC. Suppose that $\mathcal{D}$ is not equivalent to $\MECS(\mdp)$. By assumption, the ECs in $\mathcal{D}$ do not share any states. Then there exists $(\state, \action) \in \ec'$ (i.e. $(\state, \action)$ is not contained in any EC in $\mathcal{D}$) that is part of an MEC. However, we know from \Cref{lemma:state-action-mec} that $\vect{A} \vect{z} \geq \vect{1}_{\ec'}$ implies that none of the pairs in $\ec'$ are part of an MEC. \qed  
\end{proof}
Similar certificates for the MEC decomposition were also considered in \cite{jantsch_certificates_2022}, however, for our certificates the quotient does not need to be constructed.

It will also be useful to certify the \emph{absence} of satisfying ECs. This is conceptually harder, as certificates need to prove that in \emph{all} ECs the Rabin properties are violated. We now present \emph{new} certificates for this. For $i \in [k]$, we let $i \oplus 1 \coloneqq 1$ if $i = k$ and $i \oplus 1 \coloneqq i + 1$ otherwise.
\begin{definition}[Copy MDP]
Let $\mathfrak{p} = \tuple{(F_i, E_i)}_{i \in [k]}$ be a tuple of Rabin pairs and $E = \bigcap_{i=1}^k E_i$.  \todo{The way that Rabin conditions are defined, this needs to be $S \setminus \bigcup_{i=1}^k E_i$ I believe.} The \emph{copy MDP} is given by ${\mdp^\mathfrak{p}} = (E \times [k], \actions, \tuple{\init, 1}, \transMat^\mathfrak{p})$ where, for all $\tuple{\state, i}, \tuple{\state', i'} \in E \times [k]$ and $\action \in \actions(\state)$, $\transMat^\mathfrak{p}$ is defined by
\[
\transMat^\mathfrak{p}(\tuple{\state, i}, \action, \tuple{\state', i'}) =
\begin{cases}
  \transMat(\state,\action, \state') & \text{if } i = i' \land \state \notin F_i \text{ or } i \oplus 1 = i' \land \state \in F_i \\
  0 & \text{otherwise}.
\end{cases}  
\]
\label{def:copy-mdp}
\end{definition}
Intuitively, ${\mdp^\mathfrak{p}}$ consists of $k$ copies of $\mdp$ and a ``jump'' from copy $i$ to copy $i \oplus 1$ happens when a state in $F_i$ is reached.
\begin{proposition}
\label{theorem:ec-and-product-ecs}
$\ec \subseteq \SA$ is an EC of $\mdp$ with $\Conj_{i \in [k]}\ec \modelsRabin (F_i, E_i)$ if and only if there is an EC $\ec'$ of ${\mdp^\mathfrak{p}}$ such that
\begin{enumerate*}[1), itemsep=0mm, topsep=0.8mm, parsep=0mm]
\item $\ec'$ contains a state-action pair $(\tuple{\state, i}, \action)$ with $\state \in F_i$ for some $i \in [k]$
\item and $\{(\state, \action) \mid \exists i \in [k] \centerdot (\tuple{\state, i}, \action) \in \ec' \} = \ec$.
\end{enumerate*}
\end{proposition}
\begin{proof}~
\begin{itemize}
\item[$\Rightarrow$:] For states $\tuple{\state, j}$ and $\tuple{\state', j'}$ of ${\mdp^\mathfrak{p}}$, we write $\tuple{\state, j} \rightarrow \tuple{\state', j'}$ if there exists $(\state, \action) \in \ec$ such that $\transMat^\mathfrak{p}(\tuple{\state, j}, \action, \tuple{\state', j'}) > 0$. We then define $\mathsf{Reach}(\tuple{\state, j})$ to be the set of states in ${\mdp^\mathfrak{p}}$ reachable under $\rightarrow$ from $\tuple{\state, j}$.
We claim that there exists a state $\tuple{\state^*, j^*}$ such that for every $\tuple{\state', j'} \in \mathsf{Reach}(\tuple{\state^*, j^*})$ we have $\tuple{\state^*, j^*} \in \mathsf{Reach}(\tuple{\state', j'})$, that is, the states that are reachable from $\tuple{\state^*, j^*}$ can also reach it. To find such a state, we consider the following sequence of states. Let $\tuple{\state_0, j_0}$ be an arbitrary state of ${\mdp^\mathfrak{p}}$ with $\state_0 \in \states(\ec)$ and let $n = 0$.
\begin{enumerate}
\item Check whether all states in $\mathsf{Reach}(\tuple{\state_n, j_n})$ can reach it. If so, then we have found the desired state.
\item If this is not the case, then let $\tuple{\state_{n+1}, j_{n+1}}$ be a state reachable from $\tuple{\state_n, j_n}$ that cannot reach it, increment $n$ and go back to 1.
\end{enumerate}
To see that this computation eventually terminates, observe that we have 
\[
\emptyset \neq \mathsf{Reach}(\tuple{\state_{n+1}, i_{n+1}}) \subseteq \mathsf{Reach}(\tuple{\state_n, j_n}).
\]
Further, for all $0 \leq h \leq n$, we have $\tuple{\state_h, j_h} \notin \mathsf{Reach}(\tuple{\state_{n+1}, i_{n+1}})$. Otherwise $\tuple{\state_{h+1}, j_{h+1}}$ could have reached $\tuple{\state_h, j_h}$, contradicting the choice of $\tuple{\state_{h+1}, j_{h+1}}$. Thus, altogether we have
\[
\emptyset \neq \mathsf{Reach}(\tuple{\state_{n+1}, i_{n+1}}) \subseteq \mathsf{Reach}(\tuple{\state_n, i_n}) \setminus \{\tuple{\state_0, i_0}, \ldots, \tuple{\state_n, i_n}\}
\]
and we can conclude the existence of $\tuple{\state^*, j^*}$. We then define $\ec_{\mdp^\mathfrak{p}}$ by
\[
\ec' = \{ (\tuple{\state, j}, \action) \mid (\state, \action)\in \ec \land \tuple{\state, j} \in \mathsf{Reach}(\tuple{\state^*, j^*})\}.
\]
By construction, $\ec'$ is strongly connected. To see that both conditions are satisfied by $\ec'$, we note that for any state $\tuple{\state, j}$ in ${\mdp^\mathfrak{p}}$ and $\state' \in \states(\ec)$, there exists some $j'$ such that $\tuple{\state', j'} \in \mathsf{Reach}(\tuple{\state, j})$. This follows from the fact that $\ec$ is an EC and contains some state from $F_i$ for every $i \in [k]$.   
\item[$\Leftarrow$:] By assumption, we have $\ec = \{(\state, \action) \mid \exists i \in [k] \centerdot (\tuple{\state, i}, \action) \in \ec'\}$. It is easy to see that $\ec$ forms an EC in $\mdp$. Due to the first condition imposed on $\ec'$, we know that \emph{for every} $i \in [k]$, there exists $(\tuple{\state, i}, \action)$ with $\state \in F_i$. Intuitively, if $\ec'$ contains one such pair, it needs to ``go through all copies'' in order to form an EC. Together with the fact that $\ec$ only contains pairs from $\bigcap_{i=1}^k E_i$ by construction of ${\mdp^\mathfrak{p}}$, we get $\ec \models_{\mathsf{Rabin}} (F_i, E_i)$ for all $i \in [k]$.
\end{itemize}
\qed
\end{proof}
The previous theorem relates ECs that satisfy all Rabin pairs in $\mdp$ with corresponding ECs in ${\mdp^\mathfrak{p}}$. This allows us to provide a certificate for the \emph{absence} of an EC that satisfies all Rabin pairs.
\begin{theorem}
Let $\mathfrak{p} = \tuple{(F_i, E_i)}_{i \in [k]}$ be Rabin pairs and $E = \bigcap_{i=1}^k E_i$. There \emph{does not exist} an EC $\ec$ in $\mdp$ such that $\Conj_{i \in [k]}\ec \modelsRabin (F_i, E_i)$ if and only if there exists $\vect{r} \in \realsnn^{E \times [k]}$ such that for all $\state \in E$, $i \in [k]$ and $\action \in \actions(\state)$:
\[
\begin{cases}
\vect{r}(\state, i) \geq \sum_{\state' \in E} \transMat(\state, \action, \state') \cdot \vect{r}(\state', i \oplus 1) + 1 & \text{ if } \state \in F_i\\
\vect{r}(\state, i) \geq \sum_{\state' \in E} \transMat(\state, \action, \state') \cdot \vect{r}(\state', i) & \text{ otherwise }
\end{cases}
\]
A vector $\vect{r} \in \realsnn^{E \times [k]}$ is \emph{valid} for $\mathfrak{p}$ if it satisfies these inequalities.
\label{theorem:non-existence-ec}
\end{theorem}
\begin{proof}
Let $\mathfrak{p} = \tuple{(F_1, E_1), \ldots, (F_k, E_k)}$ be a tuple of Rabin pairs.
From \Cref{theorem:ec-and-product-ecs}, we know that there exists an EC $\ec$ that satisfies all Rabin pairs if and only if there exists a corresponding EC $\ec'$ in $\mdp^\mathfrak{p}$. Here, $\mdp^\mathfrak{p}$ denotes the copy MDP of $\mdp$. The \emph{system matrix} \cite{jantsch_certificates_2022} $\SM$ for $\mdp^\frak{p}$ is defined by
\[
\SM\bigl((\tuple{\state, i}, \action), \tuple{t, j}\bigr) = \begin{cases}
1 - \transMat^\mathfrak{p}(\tuple{\state, i}, \action, \tuple{t, j}) & \text{if } \state = \state' \land i = j \\
- \transMat^\mathfrak{p}(\tuple{\state, i}, \action, \tuple{t, j}) & \text{otherwise}
\end{cases}
\]
for all $\state, t \in E$, $\action \in \actions(\state)$ and $i, j \in [k]$.
Using \cite[Lemma 3.8]{jantsch_certificates_2022}, the existence of an $\ec'$ in $\mdp^\mathfrak{p}$ is equivalent to the existence of a vector $\vect{y} \in \realsnn^{\SA_{\mdp^\mathfrak{p}}}$ such that $\vect{A}^\top \vect{y} = 0$ and $\vect{t}^\top \vect{y} > 0$ where $\vect{t}(\tuple{\state, i}, \action) = 1$ if $\state \in F_i$ and $\vect{t}(\tuple{\state, i}, \action) = 0$ otherwise, for all $\state \in E$, $i \in [k]$ and $\action \in \actions(\state)$.
Consequently, there does not exist a satisfying EC if there does not exist such a solution $\vect{y}$. We then apply Farkas' lemma and obtain the following:
\begin{align*}
\neg \exists \vect{y} \in \realsnn^{\SA_{\mdp^\mathfrak{p}}} \centerdot \vect{A}^\top \vect{y} = 0 \land \vect{t}^\top \vect{y} > 0 \iff \exists \vect{r} \in \reals^{E \times [k]} \centerdot \SM \vect{r} \geq \vect{t}
\end{align*}
By writing out $\SM \vect{r} \geq \vect{t}$ explicitly, we obtain the desired certificates.
\qed
\end{proof}
Intuitively, a valid vector $\vect{r}$ certifies that there is no EC in $\mdp$ that satisfies all pairs. Now we extend this certificate to Rabin properties.
\begin{corollary}[No-EC-certificate]
Let $\pairs_1, \ldots, \pairs_k$ be sets of Rabin pairs. A \emph{valid No-EC-certificate} is a set $R$ and is \emph{valid} if for all $\mathfrak{p} \in \pairs_1 \times \cdots \times \pairs_k$ it contains $\vect{r}$ that is valid for $\mathfrak{p}$.
Then, $\mdp$ \emph{does not contain} an EC $\ec$ with $\Conj_{i \in [k]} \ec \modelsRabin \pairs_i$ if and only if there exists a valid No-EC-certificate.
\label{def:no-ec-certificate}
\end{corollary}

\todo{This set $\mathcal{R}$ is exponential, that should be discussed.}


==> omega-regular.tex <==
\section{Certificates and Witnesses for $\omega$-regular objectives}
\label{section:omega-regular}


==> reachability.tex <==
\subsection{Certificates for Reachability Queries}
\label{subsection:reachability}
Let $\mdp = (\states \union F, \actions, \init, \transMat)$ be an MDP such that $\targets$ contains all absorbing states. Further, let $\targetSets = \{\targetSet_1, \ldots, \targetSet_k\}$ where $G_i \subseteq \targets$ for all $i \in [k]$ and $\SA^* = \SA \setminus (F \times \actions)$ be the set of state-action pairs, excluding those of the absorbing states.
It was shown in \cite{baier_certificates_2024} that there exists a scheduler $\scheduler$ such that $\Conj_{i=1}^k \prob_{\mdp}^\scheduler(\eventually \targetSet_i) \geq \lambda_i$ if and only if there exists a vector $\vect{y} \in \realsnn^{\SA^*}$ such that
{ \small
\begin{align*}
&\text{for all } \state \in \states: &\initDistr(\state) + \sum\nolimits_{(\state', \action') \in \SA^*}\vect{y}(\state', \action') \cdot \transMat(\state', \action', \state) \geq \sum_{\action \in \actions(\state)} \vect{y}(\state, \action)\\
&\text{for all } i \in [k]: &\sum\nolimits_{(\state, \action) \in \SA^*} \vect{y}(\state, \action) \cdot \transMat(\state, \action, \targetSet_i) \geq \lambda_i
\end{align*}
}%
The first constraint encodes a \emph{transient flow} and the second the satisfaction of the probability thresholds. Put differently, $\vect{y}$ can also be interpreted as the expected number of times a state-action pair is seen. Crucially, a solution $\vect{y}$ can be used as a \emph{certificate}, proving the satisfaction of a query. Further, it has been shown that, for all schedulers $\scheduler$ with $\prob_{\mdp}^\scheduler(\eventually F) = 1$ we have $\Disj_{i=1}^k \prob_{\mdp}^\scheduler(\eventually \targetSet_i) \geq \lambda_i$ if and only if there exist $\vect{x} \in \realsnn^\states$ and $\vect{z} \in \realsnn^{k} \setminus \{ \vect{0} \}$ such that $\vect{x}(\init) \geq \sum_{i=1}^k \lambda_i \cdot \vect{z}(i)$ and
{ \small
\begin{align*}
\text{for all } (\state, \action) \in \SA^*: \vect{x}(\state) \leq \sum_{\state' \in \states} \transMat(\state,\action,\state') \cdot \vect{x}(\state') + \sum_{i = 1}^k \transMat(\state, \action, \targetSet_i) \cdot \vect{z}(i).
\end{align*}
}%
Note that we only quantify over schedulers that reach $\targets$ almost surely. For MDPs where all ECs are formed by states in $F$, all schedulers satisfy this property. The first constraint requires the satisfaction of the thresholds and the second encodes \emph{Bellman equations}. For more details, we refer to \cite{baier_certificates_2024}. We write $\mathcal{F}(\mdp, \mathcal{G}, \boldLambda)$ and $\mathcal{H}(\mdp, \mathcal{G}, \boldLambda)$ to denote the polyhedra formed by the inequalities for $\existsCQ$- and $\universalDQ$-reachability queries, respectively.

